Backdoor Attacks on Federated Learning with Lottery Ticket Hypothesis

Edge devices in federated learning usually have much more limited computation and communication resources compared to servers in a data center. Recently, advanced model compression methods, like the Lottery Ticket Hypothesis, have already been implemented on federated learning to reduce the model size and communication cost. However, Backdoor Attack can compromise its implementation in the federated learning scenario. The malicious edge device trains the client model with poisoned private data and uploads parameters to the center, embedding a backdoor to the global shared model after unwitting aggregative optimization. During the inference phase, the model with backdoors classifies samples with a certain trigger as one target category, while shows a slight decrease in inference accuracy to clean samples. In this work, we empirically demonstrate that Lottery Ticket models are equally vulnerable to backdoor attacks as the original dense models, and backdoor attacks can influence the structure of extracted tickets. Based on tickets' similarities between each other, we provide a feasible defense for federated learning against backdoor attacks on various datasets.

==> version_0913.tex <==
\begin{abstract}
% Deep neural networks (DNNs) achieve remarkable performance in many real-world applications, accompanied by high computation resource requirements. 
% Especially, edge devices (e.g., edge/mobile devices) in Federated learning (FL) usually have much more limited computation and communication resources compared to servers in a data center.
% Hence, many advanced model compress methods have been proposed and used towards more efficient DNNs training.
% In this work, we are the first to empirically study the robustness of the Lottery Ticket Hypothesis under the backdoor attacks.
Edge devices in Federated Learning usually have much more limited computation and communication resources compared to servers in a data center. 
Recently, advanced model compression methods, like the Lottery Ticket Hypothesis, have been proposed for more efficient DNNs training, which has already been implemented on LotteryFL. 
However, Backdoor Attack can compromise its implementation in the Federated Learning scenario. The malicious edge device trains the model with poisoned private data and uploads backdoored parameters to the center, embedding a backdoor to the global shared model after unwitting distributed optimization. During the inference phase, this backdoored model classifies samples with a certain trigger as one target category, while shows a slight decrease in inference accuracy to clean samples. In this work, we empirically demonstrate that Lottery Ticket models are equally vulnerable to the backdoor attack as the original dense models, and the backdoor attack can influence the structure of extracted sub-network. Based on these phenomena, we provide a feasible idea for Federated Learning to defend against the backdoor attack. Codes are available at \url{https://github.com/zeyuanyin/LTH-Backdoor}.
% The vulnerability of LTH has not been studied from the purview of Backdoor Attacks. In this work, we are the first to empirically demonstrate that LTH Networks are equally vulnerable to backdoor attacks as the original dense networks. %need to modify 
% LTH shows that there exist subnetworks (winning tickets) that can reach test accuracy comparable to the original network and can be trained for fewer computation resources. 
% However, the winning tickets are vulnerable to poisoning data due to the certain pruning criterion based on the training data. It is much likely that the obtained winning tickets can be infected and not achieve the expected performance if the training data is maliciously modified by the adversary. 

\end{abstract}


\section{Introduction}
\label{introduction}

Federated Learning (FL) has been proposed to address the privacy problems without direct access to sensitive training data, especially for privacy-sensitive tasks \citep{yang2019federated,kairouz2019advances}. % modified
% Federated Learning (FL) has been proposed to address the privacy problems during the training phase of machine learning models without direct access to sensitive training data, especially for privacy-sensitive tasks \citep{yang2019federated,kairouz2019advances}. % original
However, edge devices usually have much more limited computation and communication resources compared to the traditional data center, which means that the client model should be as light as possible. % modified
% However, edge devices (e.g., edge/mobile devices) in FL usually have much more limited computation and communication resources compared to servers in a data center, which means that the model running on edge devices should be as light as possible. % original
Lots of model compression methods are proposed to solve this problem \citep{han2015learning,guo2016dynamic,molchanov2016pruning,liu2018rethinking,liu2017learning}. 
One of them, the Lottery Ticket Hypothesis (LTH) \citep{frankle2019lottery}, shows that there exist subnetworks (winning tickets) that can reach test accuracy comparable to the original network with fewer computation resources usage.
\citet{li2020lotteryfl} proposed LotteryFL which applied LTH in FL scenario to alleviate the scarcity of computing resources on edge devices. 
% In terms of efficient training, \citet{frankle2019lottery,you2020drawing} study Lottery Ticket Hypothesis through the massive experiments: a dense neural network contains a subnetwork that can match the test accuracy of the original network after training for at most the same number of iterations, and the winning tickets can be drawn at very early iterations. 
Nevertheless, various security issues from the real world still need to be tackled \citep{goodfellow2014explaining,bagdasaryan2020backdoor,biggio2018wild}. 
% There are many previous works mainly focusing on adversarial attacks toward winning tickets, which are launched during the inference phase \citep{zhang2019theoretically,tsipras2018robustness,shafahi2019adversarial}. 
Backdoor attacks, which are launched during the training phase, have been recently studied on FL \citep{bagdasaryan2020backdoor,xie2019dba}.
If the attackers hack into some clients and maliciously modify their datasets, the models uploaded from the infected clients can compromise the global shared model, then the FL system will be vulnerable and may have a high risk of data leakage.

In this paper, we make LotteryFL more robust. 
% we try to trade off model accuracy, robustness, and training efficiency. 
We empirically demonstrate that Lottery Ticket model is equally vulnerable to the backdoor attack as the original dense model.
We provide detailed experiments and analysis about the phenomenon based on the theory of \citet{liu2018fine} that the backdoor attack embed backdoors in neurons or connections of neurons. 
We identify the existence of key neurons by contrasting the similarity between benign pruned models and backdoor pruned models, which helps to explain the equal vulnerability. 
Furthermore, we design a defense pattern to strengthen the robustness of the FL system.
% LTH is one of the SOTA pruning methods to train a sparse subnetwork with fewer neurons and connections than its origin network, which can make the model both slight and efficient, while the backdoor attack is to embed backdoors in neurons or connections of neurons \citep{liu2018fine}. 
% Thus, we explore the possibility of combining advanced pruning methods and backdoor defense in the model training phase to save computing resources as well as to enhance its robustness. 
% In detail, we empirically demonstrate the existence of key neurons and analyze the difference between clean pruned models $f(m\odot \theta)$ and backdoor pruned models $f^b(m\odot \theta)$.
% Then we apply this defense method to the distributed optimization process of FL to enhanced robustness of global shared models in real-world deployments. 


Our contributions are summarized as follows:
\vspace{-1em}
\begin{enumerate}
\setlength{\itemsep}{-0.5pt } 
\item We conduct various backdoor attacks on the essence of LotteryFL, Lottery Ticket Hypothesis, and demonstrate that LTH is vulnerable, which arguably shows that the backdoor attack affect winning tickets' structures and bring potential security risks to practical application.

\item We discuss the principle of backdoor embedment and the intrinsic mechanism of backdoor learning in detail, showing that neurons, retained in benign tickets, also have a high probability of being retained in attacked tickets.


\item We propose a feasible idea for LotteryFL models to detect the backdoor attack, which can develop an efficient and robust (against the backdoor attack) FL system.

\end{enumerate}

    \vspace{-1em}
\section{Related Works}
\label{related_works}
    \vspace{-0.5em}
\textbf{Lottery Ticket Hypothesis.}
% Many network pruning works have been proposed to detect and remove redundant parts of models, and keep a comparable or even better accuracy as compared to origin methods.
% \citet{han2015learning,see2016compression} propose a kind of compression method with weight pruning to prune the unimportant connections and finally retrain the network to fine-tune the weights of the remaining connections.
% \citet{liu2018rethinking} point the pruned architecture itself, rather than a set of inherited \textit{important} weights, is more crucial to the efficiency in the final model. 
% \citet{liu2017learning} propose channel pruning without the requirement for special software/hardware accelerators, which can identify and prune insignificant channels automatically.
% In terms of efficient training, 
\citet{frankle2019lottery} first demonstrate Lottery Ticket Hypothesis that there exists a small subnetwork, called the \textit{Winning Ticket}, which can make the training process more efficient and lead to a comparable accuracy to the dense network. 
\citet{liu2018rethinking} thinks that it is not necessary to inherit weight from a large model and inheriting might trap the pruned model into a bad local minimum. Based on the hypothesis, 
\citet{you2020drawing} improve the searching phase for winning tickets and propose \textit{Early-Bird Tickets} which are winning tickets can be drawn at very early iterations.

\textbf{Federated Learning.}
Federated Learning enables model training from local data collected by edge/mobile devices by uploading, downloading and aggregating model parameters, while preserving data privacy \citep{yang2019federated,kairouz2019advances}. 
In terms of accelerating FL model training, PruneFL \citep{jiang2019model} had been proposed to reduce both communication and computation overhead and minimize the overall training time with parameter pruning. 
LotteryFL \citep{li2020lotteryfl} is a personalized and communication-efficient Federated Learning framework via exploiting the Lottery Ticket hypothesis.

\textbf{Backdoor Attacks.}
Backdoor attack \citep{kairouz2019advances,chen2017targeted}, an artful kind of poison attack \citep{mei2015using,jagielski2018manipulating}, is to embed backdoors into a model by training with poisoning data.
The backdoor can hide and does not affect the performance on no-trigger data, which makes users hard to judge the existence of the backdoor only by the accuracy of the validation dataset. If the input data is with a particular trigger, the backdoor will be activated and contribute to misleading the classification result to the attack target, which will limit the using range of the model due to potential security risk.
Threats from backdoor attacks are widespread in the FL field \citep{bagdasaryan2020backdoor,xie2019dba}. 
In many practical scenarios, a minority attacked clients will embed backdoors on the FL model and disturb the FL application, which shows that FL is vulnerable to the backdoor attack.

% Current defenses against backdoor attacks mainly apply to the trained model \citep{chen2018detecting,gao2019strip,liu2019abs} and can generally be divided into three stages: detect backdoor, clean backdoor and fine-tune. \citet{wang2019neural} use reverse engineering to generate hidden triggers embedded inside deep neural networks, which can successfully defend against backdoor attack. Even if \citet{liu2018fine} add fine-pruning process to fine tune the model ensuring superior performance. However, lots of additional computation, brought by either reverse engineering or fine-tuning, counteracts the efficiency of model compress.

    \vspace{-0.5em}
\section{Approach}
\label{approach}
    \vspace{-0.5em}
% \subsection{Backdoor Attacks}
\textbf{Backdoor Attacks}
Inspired by the backdoor attack variants \citep{wang2019neural}, we use two general attack methods to evaluate the winning ticket hypothesis and our proposed defense method. 
\textit{BadNet Attack} \citep{gu2017badnets} is a classic attack with a white square trigger $k$ injected in the bottom right corner of each poisoning image. 
Besides, we design another attack form called \emph{Random Trigger Attack} by replacing the white square trigger with a random square trigger $k_{rand}$.
Taking CIFAR-10 for an example, a dataset consisting of 32$\times$32 color images with the trigger $k$ embedded at the lower-left 4$\times$4 pixels position of the picture. The outer pixels' value is set to 0, which means the pixels are invalid. After obtaining the trigger $k$, the process of generating backdoor data $x^b$ is expressed as
$x^b_{i,j}=replace(x,k)$
% =\begin{cases}
% x_{i,j}& \text{$k_{i,j}=0$}\\
% k_{i,j}& \text{$k_{i,j}\neq0$}
% \end{cases}$
where $replace(x,k)$ is used to replace pixel value of $x$ with the trigger $k$ when trigger pixel $k_{i,j}$ is valid. After generating a set of backdoor samples, we blend them with the entire benign train dataset $\mathcal{D}_{train}$ to form a malicious attack train dataset $\mathcal{D}^{b}_{train}$.


% \subsection{Attack on Winning Tickets}
\textbf{Attack on Winning Tickets}
Backdoor attacks on LotteryFL are essentially attacks on Lottery Ticket Networks, therefore we empirically evaluate the impacts of backdoor attacks on searching lottery tickets. 
We study the robustness of Early-Bird Tickets \citep{you2020drawing}, a variant of Lottery Tickets, which can be drawn at very early iterations. 
We explore the structural difference between winning tickets with and without backdoor attacks, 
and analyze the classification performance and successful backdoor attack of the attacked winning tickets.


% the combination between backdoor attacks and winning tickets on the model classification and attack success performance.

% The selection of lottery tickets is based on a criterion that important connections will be preserved and unimportant contacts will be deleted \citep{cosentino2019search, dinh2020sparsity}. 
% In terms of backdoor attacks, the signification of connections might be changed because there is poisoning data in the datasets to disturb the normal training process \citep{gao2020backdoor}. 


\section{Experiments}
\label{exp}
We use two DNN models: VGG16 \citep{simonyan2014very} and ResNet18 \citep{he2016deep}, on two common datasets: CIFAR-10/100 \citep{krizhevsky2009learning}. 
We implement two forms of backdoor attack: \emph{BadNet Attack} and \emph{Random Trigger Attack} on searching lottery tickets.

\subsection{Backdoor Attacks on the Structure of Lottery Tickets}
% \subsection{Whether Backdoor Attack Changes the Structure of Lottery Tickets?}

\begin{wraptable}{r}{0.5\textwidth}
\centering
    \vspace{-2em}
    \caption{Contrasting the similarity of different tickets' structures with the same initialization seed. Note that \textit{Backdoor (\Rmnum{1})} and \textit{Backdoor (\Rmnum{2})} represent the \emph{BadNet} and \emph{Random Trigger attacks} separately.}
    \label{similarity_of_LT}

\resizebox{0.5\textwidth}{!}{

    \begin{tabular}{cllll}
    \hline
    \multirow{2}{*}{\textbf{Setting}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Compare}}} & \multicolumn{3}{c}{\textbf{Similarity}} \\ \cline{3-5} 
     & \multicolumn{1}{c}{} & p=30\% & p=50\% & p=70\% \\ \hline
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VGG16\\ CIFAR-10\end{tabular}} & Benign - Backdoor (\Rmnum{1}) & 67.09 & 71.12 & 77.37 \\
     & Benign - Backdoor (\Rmnum{2}) & 67.52 & 72.40 & 77.98 \\ \cline{2-5} 
     & \textbf{Avg. Decrease} & \textbf{32.70} & \textbf{28.24} & \textbf{22.33} \\ \hline
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VGG16\\ CIFAR-100\end{tabular}} & Benign - Backdoor (\Rmnum{1}) & 66.62 & 75.80 & 74.29 \\
     & Benign - Backdoor (\Rmnum{2}) & 66.52 & 76.52 & 77.32 \\ \cline{2-5} 
     & \textbf{Avg. Decrease} & \textbf{33.43} & \textbf{23.84} & \textbf{24.20} \\ \hline
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}RESNET18\\ CIFAR-10\end{tabular}} & Benign - Backdoor (\Rmnum{1}) & 67.42 & 58.75 & 58.25 \\
     & Benign - Backdoor (\Rmnum{2}) & 66.54 & 59.96 & 62.13 \\ \cline{2-5} 
     & \textbf{Avg. Decrease} & \textbf{33.02} & \textbf{40.64} & \textbf{39.81} \\ \hline
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}RESNET18\\ CIFAR-100\end{tabular}} & Benign - Backdoor (\Rmnum{1}) & 79.67 & 78.04 & 75.46 \\
     & Benign - Backdoor (\Rmnum{2}) & 79.17 & 78.20 & 75.08 \\ \cline{2-5} 
     & \textbf{Avg. Decrease} & \textbf{20.58} & \textbf{21.88} & \textbf{24.73} \\ \hline
    \end{tabular}

}

\vspace{-1em}
\end{wraptable}

We conduct this attack in order to decide whether that backdoor embedment affects the lottery tickets' architecture. 
We fix the same random seeds to ensure that the setting and results of each repeated experiment are the same, so the comparison of two benign tickets obtained by repeated experiments shows 100\% similarity.
Under the setting that all random seeds are the same, we ensure that the only change in the comparison experiment is whether there is backdoor data in the dataset $\mathcal{D}_{train}$.
\tablename~\ref{similarity_of_LT} show the similarity between benign tickets and backdoor tickets. 
% to evaluate whether the structure is changed by backdoor attacks by comparing the Clean - Backdoor Similarity with the Clean - Clean Similarity. 
We observe that Benign - Backdoor Similarity is obviously lower than the Benign - Benign Similarity (100\%). Taking VGG16 with dataset CIFAR-10 under the backdoor attack (\Rmnum{1}) for example, the similarity value in the pruning 30\%, 50\%, 70\% decreases by 32.70\%, 28.24\%, 22.33\% on average respectively. 
We can conclude that the backdoor attack affect the structure of extracted lottery tickets during the searching tickets stage.


\subsection{Attacked Lottery Tickets' Performance}
% \textbf{Whether Backdoor Intensity Influences the Clean Data Accuracy?}

In this section, we evaluate the performance of backdoor-embedded lottery tickets (LT) by two indexes, Clean Data Accuracy (CDA) and Attack Success Rate (ASR), and make a comparison with benign LT. 
The CDA index is evaluated by using benign datasets to retrain the subnetworks within the poisoned lottery tickets and clean tickets. 
% A successful backdoor DNN always has a high ASR, and its CDA should be close to the benign counterpart that have little chance to be detected. 

\begin{table}[b]
    \vspace{-1em}
\centering
\caption{Clean data accuracy (CDA) and attack success rate (ASR) of different pruning rates' subnetworks structures.}
\label{preformance_of_ALT}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccccc}
\hline
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Setting}}} & \multicolumn{4}{c}{\textbf{Clean Data Accuracy (\%)}} & \multicolumn{4}{c}{\textbf{Attack Success Rate (\%)}} \\ \cline{3-10} 
\multicolumn{2}{c}{} & p=0 & p=0.3 & p=0.5 & p=0.7 \multicolumn{1}{c|}{} & p=0 & p=0.3 & p=0.5 & p=0.7 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VGG16\\ CIFAR-10\end{tabular}} & LT (benign) & 93.28 & 93.25 & 93.13 & 92.60 \multicolumn{1}{c|}{} & - & - & - & - \\
 & Backdoor (\Rmnum{1}) & 92.55 & 92.42 & 92.38 & 92.34 \multicolumn{1}{c|}{} & 95.59 & 96.36 & 96.60 & 96.69 \\
 & Backdoor (\Rmnum{2}) & 93.02 & 92.90 & 92.62 & 91.98 \multicolumn{1}{c|}{} & 100 & 100 & 100 & 100 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VGG16\\ CIFAR-100\end{tabular}} & LT (benign) & 72.04 & 71.34 & 70.53 & 69.91 \multicolumn{1}{c|}{} & - & - & - & - \\
 & Backdoor (\Rmnum{1}) & 69.97 & 69.12 & 67.73 & 63.00 \multicolumn{1}{c|}{} & 87.50 & 89.13 & 90.29 & 90.59  \\
 & Backdoor (\Rmnum{2}) & 69.48 & 68.08 & 67.93 & 64.62 \multicolumn{1}{c|}{} & 99.78 & 99.92 & 100 & 100 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}RESNET18\\ CIFAR-10\end{tabular}} & LT (benign) & 92.71 & 92.93 & 92.93 & 93.05  \multicolumn{1}{c|}{} & - & - & - & - \\
 & Backdoor (\Rmnum{1}) & 90.66 & 91.02 & 91.34 & 90.06 \multicolumn{1}{c|}{} & 97.28 & 97.33 & 97.35 &  97.22  \\
 & Backdoor (\Rmnum{2}) & 91.13 & 89.89 & 90.51 & 90.18 \multicolumn{1}{c|}{}& 100 & 100 & 100 & 100 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}RESNET18\\ CIFAR-100\end{tabular}} & LT (benign) & 71.59 & 71.45 & 70.94 & 70.04  \multicolumn{1}{c|}{} & - & - & - & - \\
 & Backdoor (\Rmnum{1}) & 69.46 & 68.60 & 67.11 & 65.04 \multicolumn{1}{c|}{} & 89.03 & 87.59 & 89.73 & 89.67  \\
 & Backdoor (\Rmnum{2}) & 70.02 & 69.52 & 67.58 & 66.58 \multicolumn{1}{c|}{} & 99.80 & 99.65 & 99.24 & 99.86  \\ \hline
\end{tabular}%
}
    \vspace{-1em}
\end{table}

% \subsection{Backdoor lottery tickets' }
% We consider a real-world scenario where researchers unknowingly use the backdoor datasets to train their models using EB Train, an efficient training of deep networks mentioned above. Researchers will use the backdoor datasets to search for winning tickets, prune the structures and retrain the subnetworks.

We draw two main conclusions from the experiment data in \tablename~\ref{preformance_of_ALT}.
First, comparing the CDA of benign LT with attacked LT at the same pruning rate, we find that the latter is not significantly different from the former. For example, the CDA of Backdoor(\Rmnum{1}) is only 0.83\% lower than the benign LT. It shows that backdoor DNNs can reduce the likelihood of being detected. 
Second, comparing the difference in ASR between dense network $(p=0)$ and pruned network $(p>0)$ under the same attack, we find that there is high ASR in both dense and pruned networks, which indicates that the lottery ticket networks are equally vulnerable to backdoor attacks as the original dense networks.

\vspace{-1.75em}
\subsection{Discussion}
\label{discussion}
\vspace{-0.5em}
\textbf{The Existence of Key Neurons.}
According to the first finding above, we suppose that some key neurons with decisive roles on the CDA index will be preserved whether or not backdoors embedded into DNNs. This is corresponding to the Neural Architecture Search (NAS) which is to find the optimal network structure in dense models. To illustrate this supposition, \figurename~\ref{visualize} plots the distribution of pruned neurons between the clean model $f(\theta)$ (trained by benign datasets $\mathcal{D}$), and backdoor model $f^b(\theta)$ (trained by backdoor datasets $\mathcal{D}^{b}$). Green squares and red squares represent the neurons retained in $f(m\odot \theta)$ and $f^b(m\odot \theta)$, respectively, where $m$ is a mask. Yellow squares stand for neurons that are both retained, and pale squares stand for neither retained.
As shown in \figurename~\ref{visualize}, yellow squares, standing for both-retained neurons, occupy most of the position.
We can conclude that neurons that are retained in $f(m\odot \theta)$ also have a high probability of being retained in $f^b(m\odot \theta)$, thus the embedment of backdoors does not significantly compromise the model's CDA index. In the appendix \ref{appendix:key_neurons}, we carry out further experiments to demonstrate how these both-retained neurons have decisive roles in the inference phase by precise figures.


\begin{figure}[t]
    \vspace{-2em}
    \centering
    \includegraphics[width=1\textwidth]{figure/HeatMap.pdf}
        \vspace{-2em}
    \caption{Visualization of the  distribution heat map of retained neurons in $[0, 5, 12]^{th}$ layers between the normal model $f(m \odot \theta)$ and backdoored model $f^b(m\odot \theta)$ on CIFAR-10 where $p$ = 0.3.}
    \label{visualize}
    \vspace{-1.7em}
\end{figure}

% In conclusion, backdoor attacks actually have an influence on drawing EB tickets according to Table~\ref{preformance_of_ATL}. The influence is mainly on indecisive neurons, but is too slight to deviate the key neurons, which explains the following retraining process to train a sparse model almost causes no extra loss of accuracy. Even the intensity of attacks has been strengthened, the subnetworks' performance by retraining with benign datasets is not decreasing obviously. We come up with some possible reasons: 1) neurons and connections that play a leading role in the network account for a small proportion and are preserved in both normal subnetworks and backdoor subnetworks; 2) the subnetworks after channel pruning are as deep as the dense networks and also have a strong learning ability; 3) retraining for a large number of epochs enable the network to achieve great accuracy.

% % \vspace{-1.0em}
% \textbf{Efficiency and Robustness.} 
% We notice that backdoors can mysteriously embed in key neurons and achieve the attack due to the experimental result that the channel pruning technical can hardly disable the effect of backdoor attack. Although models can be trained more efficiently, the model is also vulnerable to backdoor attacks. Previous works have proposed some defense which is not effective in real world scenarios. 
% Fine-pruning \citep{liu2018fine} prunes the backdoor-sensitive neurons, which has an irreversible impact on the CDA performance because backdoors are mixed with key neurons. And the fine tuning process would consume more computing resources. There is a promising research field to seek the bridge between both efficiency and robustness.

\input{algorithm}

\textbf{Defense on Federated Learning with Lottery Tickets Hypothesis.}
According to the larger difference on similarity between benign tickets and backdoor tickets than difference among benign tickets, we propose a backdoor detection algorithm \textbf{Detect()} to detect whether a client ticket is a backdoor ticket. $\mathcal{L} \in R^k$ denotes a boolean vector, where $\mathcal{L}[i] = true$ represents the detected backdoor ticket $\theta_i$ and $\mathcal{L}[i] = false$ represents the benign ticket $\theta_i$.
We use \textbf{FineTune()} to train the detected backdoor tickets $\theta_i[\mathcal{L}]$ for some epochs on server-own validation data, based on the effective fine-tuning process in \citep{liu2018fine}.
For specific LotteryFL functions shown on Algorithm~\ref{algorithm}, \textbf{Prune()} outputs the mask $m_i$ by pruning $\theta_i$ at the pruning rate $r_p$. 
\textbf{ClientUpdate()} receives weights from edge devices. 
\textbf{AggregateLTNs()} is weight aggregation process, like FedAvg \citep{mcmahan2017communication}.
% and aggregate some advanced backdoor pruning methods 
% \citep{liu2018fine} to form an integral defense on Federated Learning using Lottery Tickets. 

\vspace{-1em}
\section{Conclusion and Future Work}
\label{conclusion}
\vspace{-0.5em}
In this paper, we are the first to demonstrate the LotteryFL is as vulnerable to backdoor attacks as the origin FL and analyze in detail that the ticket's structure can be affected by the attack while most decisive neurons still retain under the attack. We further provide an integral defense algorithm on LotteryFL. 
There are promising research directions in the future: 1) robustness of LotteryFL should be evaluated by more advanced backdoor attacks; 2) robustness in the case of label deficiency of LotteryFL should be enhanced in the future.



% From the perspective of backdoor attacks, there should be more advanced backdoor attack methods \citep{saha2020hidden,li2020invisible,doan2020februus,liao2018backdoor} that are used to test the efficient model's robustness and fine-tuning defense framework's validation. 

